In-Context Prompt Editing For Conditional Audio Generation

Distributional shift is a central challenge in the deployment of machine learning models as they can be ill-equipped for real-world data. This is particularly evident in text-to-audio generation where the encoded representations are easily undermined by unseen prompts, which leads to the degradation of generated audio -- the limited set of the text-audio pairs remains inadequate for conditional audio generation in the wild as user prompts are under-specified. In particular, we observe a consistent audio quality degradation in generated audio samples with user prompts, as opposed to training set prompts. To this end, we present a retrieval-based in-context prompt editing framework that leverages the training captions as demonstrative exemplars to revisit the user prompts. We show that the framework enhanced the audio quality across the set of collected user prompts, which were edited with reference to the training captions as exemplars.

==> sections/3_analysis.tex <==



Audio generation models are trained with a distribution of captions; whereas user prompts are often under-specified and differ from this distribution. Probing music models with a diverse set of prompts consisting of words/phrases coming from user prompts, training set, and their combinations allows us to understand their interactions and most importantly, answering the first research question,

RQ1: which distribution of prompts makes better music?

The answer to RQ1 allows us to better construct an in-context learning setup since we can then rank and select exemplars prompts, leading to the second question,

RQ2: How can we select and rank training captions as exemplars for in-context learning?

Lastly, we want to explore soft and iterative prompting using an additional text encoder that generates and regenerates latent code z where each iteration results in a music sample, which we then obtain a quality signal on this sample, and then decide if iteration should be stopped.
This led to two additional questions,

RQ3: How do we train “soft prompter” ?

RQ4: How do define the right automatic quality metrics for audio samples that can improve soft prompters and also as terminating conditions?





==> sections/algorithm.tex <==

\begin{algorithm}[htb]
\vspace{0.1cm}
	\caption{Feedback Instruction Learning}
	\label{alg:feedback}
		\begin{algorithmic}[1]
		    \STATE \textbf{Input:}
      Prompt set $\cX=\{x_1,\ldots,x_n\}$, reward function $r(\cdot)$, initial model $G_0 = g(w_0,\cdot)$, acceptance ratio $1/k$, batch size $b$, temperature parameter $\alpha$. %$\lambda$.
			\FOR{Stage $t=1,\dots,T$}
			\STATE {\color{teal} \textbf{\textit{1 . Data collection.}}} Sample a batch $\mathcal{D}_t$ from $\cX$ of size $b$;
            \FOR{$x \in \mathcal{D}_t$}
			\STATE 
            Generate $y \sim p^{\alpha}_{G_{t-1}}$ and compute $r(x,y)$.
             \ENDFOR
    % \STATE {\color{teal} \textbf{\textit{2. Data ranking.}}} Let $\cB$ be the $\lfloor b / k\rfloor$ samples with maximum rewards; 
   % \STATE {\color{teal} \textbf{\textit{3. Model fine-tuning.}}} Fine-tune $w_{t-1}$ on $\cB$ to obtain $G_t = g(w_{t}, \cdot)$.
			\ENDFOR
		\end{algorithmic}
\vspace{0.1cm}
\end{algorithm}


==> sections/inst_template.tex <==

\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.3\linewidth} p{0.2\linewidth}p{0.5\linewidth}}
\toprule
\textbf{User Input} & \textbf{ Instruction} & \textbf{Enhanced Prompt} \\
\midrule
\emph{Write a detailed description describing the music with instruments, tone, pitch, rhythm, atmosphere, style, and all the audio details.}

& \emph{Rewrite the following prompts to be diverse and different}

& \emph{1. Describe the instruments used in the music, including their tone, pitch, and rhythm. 2. Provide details about the overall sound and atmosphere of the music, including the style and genre. 3. Include any special effects or layers that enhance the music, such as layers of guitars or synths.} \\
% \hdashline
\bottomrule
\end{tabular}}
\caption{\small The provided example represents a pair of instruction-input and output generated by instruction-tuned LLMs.}\label{tab:example}
\end{table*}

==> sections/instruction_example.tex <==

\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.15\linewidth} p{0.4\linewidth}p{0.45\linewidth}}
\toprule
\textbf{User Input} & \textbf{ Instruction} & \textbf{Enhanced Prompt} \\
\midrule
\emph{Cupcake}

& \emph{Write a detailed description describing the music with instruments, tone, pitch, rhythm, atmosphere, style, and all the audio details.}

& \emph{The music for the cupcake video is upbeat and cheerful, featuring a mix of bouncy electronic elements and live instruments such as guitar and drums. The tone is light and playful, with a catchy melody and a steady beat that evokes feelings of happiness and joy.} \\
% \hdashline
\bottomrule
\end{tabular}}
\caption{\small The provided example represents a pair of instruction-input and output generated by instruction-tuned LLMs.}\label{tab:example}
\end{table*}

==> sections/instruction_format.tex <==

\begin{figure}[h]
  \centering
\includegraphics[width=0.6\columnwidth]{emnlp2023-latex/diagrams/instruction_format_v2.pdf}
\caption{ \small  The provided example represents a pair of instruction-input and output that is utilized to train instruction-tuned LLMs.
}
\label{fig:instruction}
\end{figure}


==> sections/table1.tex <==


\begin{table}[hb]
  \small
\centering
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{lcccccccc}
    \toprule
    & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen \\ 
    \midrule
% \text{Number of instances} & 40                                                        & 20                                   & 100                                   & 25                                   & 25                                    & 25                                    & 25                                    & 40                                    \\ 
\text{Average number of cells}        & 168.85                                                        & 74.90                                   & 39.46                                   & 27.92                                   & 12.56                                    & 27.6                                   & 34.0                                     & 52.25                                    \\ 
\text{Average number of cells (DL)}          & 3.26                                                        & 2.05                                   & 2.24                                   & 2.44                                   & 3.16                                    & 2.36                                    & 1.68                                     & 2.68                                    \\ 
\text{LS}               & 0.60                                                        & 0.58                                   & 0.59                                   & 0.63                                   & 0.60                                    & 0.61                                    & 0.62                                     & 0.62                                    \\ 
\text{MSTTR}            & 0.56                                                        & 0.60                                   & 0.58                                   & 0.59                                   & 0.60                                    & 0.61                                    & 0.56                                     & 0.61                                    \\ 
 \bottomrule
\end{tabular} }
\caption{ \small caption.}
\label{corpus_stats}
\end{table}
